SyncVid: World-Equivariant Diffusion for Synchronized Video Generation

Generating multiple videos of a dynamic scene from a single reference video requires synthesizing both observed and unobserved content consistently across viewpoints. Existing camera-control methods for video diffusion typically rely on architectural mechanisms, including camera embeddings, cross-view attention, and geometric conditioning. Although effective for static scene content, these approaches often struggle with the fine-grained, dynamic geometry that must remain coherent across views and over time. We synchronize the diffusion process itself by sampling the Gaussian noise prior in a canonical 3D space derived from the source video and rasterizing it into target cameras, rather than sampling independently in each 2D image plane. Our method, SyncVid, lifts a monocular video into a canonical 4D representation, associates noise with scene geometry and unseen space, and rasterizes the resulting structured noise into arbitrary views. Because rendering can introduce local correlations, we further propose a cross-view-consistent whitening procedure that decorrelates neighboring pixels while preserving correspondence across views. The structured noise serves as the diffusion prior for a LoRA-adapted pretrained video diffusion model, requiring no architectural modifications. By enforcing spatiotemporal and cross-view coherence at the source of stochasticity, SyncVid generates synchronized videos and improves both perceptual quality and cross-view consistency in our experiments. Project page: https://qualcomm-ai-research.github.io/SyncVid-Webpage.

==> floats/tables/denoising_steps.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Effect of the number of denoising steps} used at inference time for the Wan2.2-5B backbone (Sec.~\ref{sec:denoising_steps}). \textbf{Bold} marks the setting used in all other experiments.}
\label{tab:denoising_steps}
\begin{tabular}{cccccc}
\toprule
Steps & Mat.\ Pix.\,(K) $\uparrow$ & CLIP-V $\uparrow$ & CLIP-F $\uparrow$ & Rot.\ Err.\,($^\circ$) $\downarrow$ & Trans.\ Err. $\downarrow$ \\
\midrule
15           & 1571.75                   & 90.14 & 97.41 & 7.91 & 0.67 \\
\textbf{20}  & \textbf{1607.35}           & 90.31 & 97.39 & 8.35 & 0.56 \\
30           & 1514.93                   & 90.44 & 97.47 & 8.54 & 0.54 \\
50           & 1544.21                   & 90.52 & 97.40 & 8.14 & 0.60 \\
100          & 1541.44                   & 90.03 & 97.18 & 7.50 & 0.55 \\
\bottomrule
\end{tabular}
\end{table}


==> floats/tables/wrs_results.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{World Recovery Score} on a test OpenSora scene (Sec.~\ref{sec:world_recovery_score}), mean $\pm$
  standard deviation over the scene's frames.}
  \label{tab:wrs_results}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{lcccc}
  \toprule
  Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & DINO $\uparrow$ \\
  \midrule
  DaS~\cite{gu2025das}                               & 14.44 \textcolor{gray}{$\pm$ 3.22}          & 0.495 \textcolor{gray}{$\pm$ 0.156}          & 0.599 \textcolor{gray}{$\pm$ 0.109}          & 0.619 \textcolor{gray}{$\pm$ 0.181} \\
  Go-with-the-Flow~\cite{burgert2025gowiththeflow}   & 14.90 \textcolor{gray}{$\pm$ 3.04}          & 0.515 \textcolor{gray}{$\pm$ 0.154}          & 0.567 \textcolor{gray}{$\pm$ 0.111}          & 0.695 \textcolor{gray}{$\pm$ 0.173} \\
  ReCamMaster~\cite{bai2025recammaster}              & 15.02 \textcolor{gray}{$\pm$ 2.96}          & 0.524 \textcolor{gray}{$\pm$ 0.154}          & 0.579 \textcolor{gray}{$\pm$ 0.092}          & 0.677 \textcolor{gray}{$\pm$ 0.148} \\
  Reshoot-Anything~\cite{paliwal2026reshootanything} & 17.28 \textcolor{gray}{$\pm$ 3.53}          & 0.581 \textcolor{gray}{$\pm$ 0.152}          & 0.458 \textcolor{gray}{$\pm$ 0.131}          & 0.788 \textcolor{gray}{$\pm$ 0.165} \\
  ArtiFixer~\cite{delutio2026artifixer}              & 17.42 \textcolor{gray}{$\pm$ 3.57}          & 0.587 \textcolor{gray}{$\pm$ 0.159}          & 0.455 \textcolor{gray}{$\pm$ 0.133}          & 0.802 \textcolor{gray}{$\pm$ 0.145} \\
  \textbf{Ours}                                      & \textbf{--}               & \textbf{--}                & \textbf{--}                & \textbf{--}       \\
  \bottomrule
  \end{tabular}}
\end{table}

